A topological description of loss surfaces based on Betti Numbers

In the context of deep learning models, attention has recently been paid to studying the surface of the loss function in order to better understand training with methods based on gradient descent. This search for an appropriate description, both analytical and topological, has led to numerous efforts to identify spurious minima and characterize gradient dynamics. Our work aims to contribute to this field by providing a topological measure to evaluate loss complexity in the case of multilayer neural networks. We compare deep and shallow architectures with common sigmoidal activation functions by deriving upper and lower bounds on the complexity of their loss function and revealing how that complexity is influenced by the number of hidden units, training models, and the activation function used. Additionally, we found that certain variations in the loss function or model architecture, such as adding an $\ell_2$ regularization term or implementing skip connections in a feedforward network, do not affect loss topology in specific cases.

==> sections/old.tex <==

% We show here a simple example that suppose, we have $4$ layers and the last layer is linear: $f_{\theta}(x) = a^4 \in \mathbb{R}$ and we want ot compute $\frac{\partial{a^4}}{\partial w^1_{1,1}}$.
% This is equivalent to use Equation \ref{degree_on_delta_l} with the function $\mathcal{L} $ equal to the identity, in this case $\delta^4=1$.
% Now 
% \begin{align*}
%     \delta^4 &= 1\\
%     \delta^3 &= \delta^4 W^4 \sigma(a^3) \\
%     \delta^2 &= \delta^3 W^3 \sigma(a^2) \\
%     \delta^1 &= \delta^2 W^2 \sigma(a^1) \\
% \end{align*}

% We know that $\frac{\partial{a^4}}{\partial w^1_{1,1}}= \delta_1^1 x_1 $
% \begin{equation*} \frac{\partial a^4_h}{\partial w_{i,j}^{1}} = 
% \tikz[baseline]{\node(d4) {$W_h^{4}$}}(   \tikz[baseline]{\node(d5){$W^{3}$}} (( \tikz[baseline]{\node(d6) {$W^{2}_i$}}  \tikz[baseline]{\node(d7){$\sigma'(a^1_i)x_j $}} )\odot \tikz[baseline]{\node(d8){$\sigma'(a^{2}))$}} \odot \tikz[baseline]{\node(d9)
% {$\sigma'(a^{3} )$}})
% \end{equation*}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[ultra thin, ->] (d4) to [in=90,out=265] + (225:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{1 \times n_3}$};
% \draw[ultra thin,->] (d5) to [in=90,out=265] +(235:1.8cm) node[anchor=north,text = black] {$\in \mathbb{R}^{n_3 \times n_2}$};
% \draw[ultra thin,->] (d6) to [in=90,out=265] +(270:2.3cm) node[anchor=north,text = black,text width=3cm,align=center]
%  {$\mathbb{R}^{n_2 }$};
% \draw[ultra thin,->] (d7) to [in=90,out=265] +(290:1.4cm) node[anchor=north,text = black,text width=3cm,align=center]
%  {$\mathbb{R}$};
% \draw[ultra thin, ->] (d8) to [in=90,out=265] + (295:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{n_2}$};
% \draw[ultra thin, ->] (d9) to [in=90,out=265] + (300:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{n_3 }$};
% \end{tikzpicture} \newline \newline\newline\newline\newline






% \textcolor{red}{PARTE VECCHIA}

% \begin{lemma}[``Pfaffianity''of the network function wrt the parameters] \label{lem:network_pfaf}




% Let $\sigma: \mathbb{R} \rightarrow \mathbb{R}$ be a function for which there exists a Pfaffian chain $c= ( \sigma_1, \dots, \sigma_{\ell})$ and $\ell +1$ polynomials,  $Q$  and $P_i$, $1 \leq i \leq \ell$ of degree $\beta$ and $\alpha$, respectively, s.t. :

% $$ \frac{\partial \sigma_i(a)}{\partial a}  = P_i(a, \sigma_1(a), \dots, \sigma_i(a)), \; \; 1 \leq i \leq \ell$$
% $$ \sigma(a) = Q(\sigma_1(a), \dots, \sigma_{\ell} (a)) $$

% Moreover, let $g: \mathbb{R} \rightarrow \mathbb{R}$ be a function for which there exists a Pfaffian chain $( g_1, \dots, g_{\ell_{o}})$ and $\ell_{o} +1$ polynomials,  $Q_g$  and $P_g^i$, $1 \leq i \leq \ell$ of degree $\beta_g$ and $\alpha_g$, respectively, s.t. :

% $$ \frac{\partial g_i(a)}{\partial a}  = P_g^i(a, g_1(a), \dots, g_i(a)), \; \; 1 \leq i \leq \ell_{o}$$

% $$ g(a) = Q_g(g_1(a), \dots, g_{\ell_{o}} (a)) $$

% Let $f(\theta,x )$ be the function implemented by a neural network with parameters $\theta \in \mathbb{R}^n$, input $x \in \mathbb{R}^{n_0}$ and activation function $\sigma$ for all layers except  the last. The last layer can be either have activation function $g$ or be linear.
% We denote $n$ as the total number of parameters in the neural network $n=\sum_{k=1}^N n_k \cdot n_{k-1}$. 
% Let us consider the case of a real output, i.e. $f : \mathbb{R}^n \rightarrow \mathbb{R}$.
% Then, $f(\theta,x )$ is Pfaffian with complexity bounded by $ ((L-2)( \beta + \alpha  + \alpha (\beta + 1) ) + \beta , \; \; \beta + 1, \; \;  \ell h  (L-1)  )$ when $f(\theta,x ) = a^L$ and $((L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \; \; \beta_g , \; \;  \ell h ( L- 1) + \ell_{o}    )$ if $f(\theta,x ) = g(a^L)$.

% \end{lemma}




% \begin{remark}

% If the activation function is the sigmoid function, $\ell =1$, $ \alpha = 2$ and $\beta = 1$.
% So, if  the last layer is linear, when the network is shallow ($L=2$) the complexity is bounded by $ ( 1 , \; \; 2, \; \;  h )$ while when the network is deep ($L>2$) the complexity is bounded by $ (7(L-2) + 1 , \; \; 2, \; \;  h  (L-1)  )$. 
% It is clear that in the deep case a dependency on the number of layers comes up, as it is naturally expected (and confirming the previous results by \cite{bianchini2014complexity}). Nevertheless, this result is not the same found in that work, as we verify the Pfaffianity of the network w.r.t. the weights. 
% \end{remark}

% \begin{proof}\label{proof:network_pfaf}
% If the last layer is linear, $f_{\theta}(x) = a^L$, otherwise if we apply the non linearity to the last layer (for instance in the case of binary classification) $f_{\theta}(x) = g(a^L)$.
% To prove this theorem  let's start with the case where the last layer is linear, we will use eq \ref{degree_on_delta_l} with the function $\mathcal{L} $ equal to the identity. 

% For the general term $a_l$ we have distinct cases:

% $$\frac{\partial a^l_h}{\partial w_{j}^l} = \delta_{h,j} z_j^{l-1} $$
% while 
% $$\frac{\partial a^{l+1}_h}{\partial w_{i,j}^{l}} =  W^{l+1}_{h,i} \sigma'(a^l_i)z_j^{l-1} 
% $$


% $$\frac{\partial a^{l+2}_h}{\partial w_{i,j}^{l}} = W^{l+2}_h(W^{l+1}_i \sigma'(a^l_i)z_j^{l-1} ) \odot \sigma'(a^{l+1}))
% $$

% In general, for $l $ s.t. $k-l \geq 3$ 
% $$\frac{\partial a^k_h}{\partial w_{i,j}^{l}} = W_h^{k}( W^{k-1}(\dots( W^{l+2}_h(W^{l+1}_i \sigma'(a^l_i)z_j^{l-1} ) \odot \sigma'(a^{l+1})) )\dots )\odot \sigma'(a^{k-2} ) \odot \sigma'(a^{k-1}))=
% $$


% $$\frac{\partial a^k_h}{\partial w_{i,j}^{l}} = W_h^{k} \{ [W^{k-1}(\dots(\frac{\partial a^{l+2}_h}{\partial w_{i,j}^{l}} )\dots )\odot \sigma'(a^{k-2} ) ] \odot \sigma'(a^{k-1}) \}
% $$

% (example to understand better how this work ):
% \begin{equation*} \frac{\partial a^4_h}{\partial w_{i,j}^{1}} = 
% \tikz[baseline]{\node(d4) {$W_h^{4}$}}(   \tikz[baseline]{\node(d5){$W^{3}$}} (( \tikz[baseline]{\node(d6) {$W^{2}_i$}}  \tikz[baseline]{\node(d7){$\sigma'(a^1_i)x_j $}} )\odot \tikz[baseline]{\node(d8){$\sigma'(a^{2}))$}} \odot \tikz[baseline]{\node(d9)
% {$\sigma'(a^{3} )$}})
% \end{equation*}

% \begin{tikzpicture}[remember picture,overlay]
% \draw[ultra thin, ->] (d4) to [in=90,out=265] + (225:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{1 \times n_3}$};
% \draw[ultra thin,->] (d5) to [in=90,out=265] +(235:1.8cm) node[anchor=north,text = black] {$\in \mathbb{R}^{n_3 \times n_2}$};
% \draw[ultra thin,->] (d6) to [in=90,out=265] +(270:2.3cm) node[anchor=north,text = black,text width=3cm,align=center]
%  {$\mathbb{R}^{n_2 }$};
% \draw[ultra thin,->] (d7) to [in=90,out=265] +(290:1.4cm) node[anchor=north,text = black,text width=3cm,align=center]
%  {$\mathbb{R}$};
% \draw[ultra thin, ->] (d8) to [in=90,out=265] + (295:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{n_2}$};
% \draw[ultra thin, ->] (d9) to [in=90,out=265] + (300:2.7cm) node[anchor=north,text = black] {$ \in \mathbb{R}^{n_3 }$};
% \end{tikzpicture} \newline \newline\newline\newline\newline

% Now, if $y_i = \sigma_i(a)$: 
% \begin{equation*}
%     \frac{d \sigma(a)}{d a} \bigg|_{a = a_h^l} =  \frac{ d Q(y_1, \dots, y_{\ell} )}{d a}\bigg|_{a = a_h^l} =  \Big(  \sum_{s= 1}^\ell \frac{\partial Q(y_1, \dots, y_\ell) }{\partial y_{s}} P_u(a, y_1, \dots, y_u) \Big) \bigg|_{
%  \begin{array}{c}
%       1\leq u \leq \ell \\
%       y_u = \sigma_u(a_h^l) \\ 
%       a = a_h^l
%  \end{array} }
% \end{equation*}

% $\frac{\partial Q(y_1, \dots, y_\ell) }{\partial y_{s}} $ has degree $ \beta - 1$ and $P_u(a, y_1, \dots, y_u)$ has degree $\alpha $ in $\sigma_1(a), \dots, \sigma_{\ell}(a)$. In conclusion $  \frac{d \sigma(a)}{d a} \bigg|_{a = a_h^l}  $ is a polynomial of degree $ \beta  + \alpha - 1 $ if, $\forall i $, $P_i$ does not depend directly on $a$, and it is  $ \beta  + \alpha - 1 + \alpha (\beta +1) $ in the general case.

% Indeed if $P_i$ depends on $a$, we have that $P(a_h^l, \sigma_1(a_h^l), \dots, a_h^l)$ has degree $\alpha(\beta +1)$, since the degree of $a_h^l $ is $\beta +1 $ in the Pfaffian chain. 
% Notice that $a_h^l= W^l \sigma(a^{l-1})$ and $\sigma(a^{l-1})$ has degree $\beta $.


% %in
% %$( \sigma_1(a_h^l), \dots, \sigma_{\ell}(a_{h}^l))$. 

% As a consequence $ a^{\tilde{l}}_{\tilde{h}}$ is Pfaffian with respect to the chain constructed by applying all the 
% $\sigma_i, 1 \leq i \leq \ell$
% , on all the activation levels $a^k_h$ of neuron 
% $j$ in layer $k$) up to layer $\tilde{l} -1 $:
%  $ ( \sigma_1(a_1^1), \dots, \sigma_{\ell}(a_1^1), \sigma_{1}(a_2^1), \dots,  \sigma_{1}(a_{n_L}^L)), \dots , \sigma_{\ell}(a_1^1) $ (nel nostro caso $n_L =1$).
 
 
 
%  %is polynomial w.r.t. the chain $ ( \sigma_1(a_1^1), \dots, \sigma_{\ell}(a_{n_L}^L))$ (nel nostro caso $n_L =1$).
% % \textbf{vedere Lemma 2 loro, perché non dipende dai layer?} Io direi che nel nostro caso la lunghezza della catena è $\ell \times h \times (L-1) $
% % \textcolor{red}{Sì amò è sensato perchè nel nostro caso prendiamo la loss rispetto ai pesi, non rispetto all'input}

% It follows that
% $$\frac{\partial a^{l+2}_h}{\partial w_{i,j}^{l}}$$ is a polynomial (w.r.t. the chain above and the parameters) whose degree is (in the case $k-l >3$), $ (k -(l+1)) +  [(k - 1-l)( \beta + \alpha - 1 + \alpha( \beta+1))]  + (\beta + 1)  $.
% % The maximum degree is 
% %$ (L-2)^2 ( \beta + \alpha -1 + \alpha (\beta+1)) + \beta +1 $ 
% % (fare la stessa distinzione loro del lamma quando $P_i$ dipende da $a$ oppure no).



% % Da cancellare poi. analizziamo da dove vengono questi termini:
% \begin{equation*} 
% \tikz[baseline]{\node(d1) {$(k -(l+1))$}} + \tikz[baseline]{\node(d2){$[(k - 1-l)( \beta + \alpha - 1 + \alpha (\beta+1))]$}}  \tikz[baseline]{\node(d3){$+ \beta $}} 
% \end{equation*}

% % \begin{tikzpicture}[remember picture,overlay]
% % \draw[ultra thin, ->] (d1) to   [in=90,out=265] + (225:1.1 cm) node[anchor=north,text = black] {dai pesi moltiplicati  \\ tra loro, i W};
% % \draw[ultra thin, ->] (d2) to  [in=90,out=265] + (260:1.7 cm) node[anchor=north,text = black] {dai g' moltiplicati tra loro};
% % \draw[ultra thin, ->] (d3) to  [in=90,out=265] + (270:1.1 cm) node[anchor=north,text = black] {da $z^{l-1}$};
% % \end{tikzpicture} \newline \newline \newline \newline



% $a^l$ can be expressed as a polynomial in 
% $ ( \sigma_1(a_1^1), \dots, \sigma_{\ell}(a_1^1), \sigma_{1}(a_2^1), \dots,  \sigma_{1}(a_{n_L}^L)), \dots , \sigma_{\ell}(a_1^1) $ and the weights and the 
% degree of the polynomial is $\beta +1 $ since $a^l = W^l z^{l-1}$.

% So $f(\theta,x )$ is Pfaffian with complexity 
% $$ ((L-2) + (L-2)( \beta + \alpha -1 + \alpha (\beta + 1) ) + \beta , \; \; \beta + 1, \; \;  \ell h  (L-1)  )$$.
% $$ = ((L-2)( \beta + \alpha  + \alpha (\beta + 1) ) + \beta , \; \; \beta + 1, \; \;  \ell h  (L-1)  )$$


% If $ f(\theta, x) = \sigma(a^L)$:
% $$\frac{ \partial{f(\theta, x)}}{\partial w_{i,j} }= \sigma'(a^L) \frac{\partial a^L}{\partial w_{i,j}^{l}}.$$
% So the complexity of the chain is 
% $$ ((L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \; \; \beta , \; \;  \ell h ( L- 1) + \ell    )$$
% % (Aggiungo un 1 al grado dei polinomi delle derivate e $\ell$ termini alla catena, visto che ho anche $\sigma_1(a^L), \dots,  \sigma_{\ell}(a^L)$.


% If $ f(\theta, x) = g(a^L)$:
% $$\frac{ \partial{f(\theta, x)}}{\partial w_{i,j} }= g'(a^L) \frac{\partial a^L}{\partial w_{i,j}^{l}}.$$
% So the complexity of the chain is 
% $$ (\max\{(L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \beta_o + \alpha_o -1 + \alpha_o(\beta_o +1) \}, \; \; \beta_o , \; \;  \ell h ( L- 1) + \ell_o    )$$

% Indeed, we take the maximum between $(L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1$ and $\beta_o + \alpha_o -1 + \alpha_o(\beta_o +1)$  for the first term of the triplets; moreover, the length of the chain increments with $\ell_o$ terms, since we have to take in account also $g_1(a^L), \dots,  g_{\ell_o}(a^L)$.

% \end{proof}

% % Possiamo scrivere in complessità della catena

% % The degree of the poly is $k-l$, so is max when $k = L $ and $l = 1$. In this case the degree is : $L-1$
% % And considering that $ f(\theta,x^t) = a^L $ we obtain that the Loss is a pfaffian function  wrt to the weights wrt the following chain that contains all possibles 
% % $$
% %  ( g(a_{i}^l)_k, \; g'(a_j^m)_h)
% %  \; \textrm{ for } i,j  \in \{ 1, \dots n_l \}, \;  l, m  \in \{ 1, \dots , L\} , \;  
% %  h,k  \in \{ 1, \dots , m\}$$


% % $\alpha$ will be the maximum from the number of elements of the chain involved in the derivative $\frac{\partial \mathcal{L}}{\partial w_{i,j}^l}$ (which is $2 \cdot (L-l+1)$, where its maximum, when $l=1$, is $2\cdot L$) and the maximum degree for $\frac{\partial{g(a_h^k)}}{\partial w_{i,j}^l}$, which is $L$, is eventually $2\cdot L$. 
% % Therefore, $\alpha = 2 \cdot L$.
  

% % The triplet of the chain $(\alpha, \beta, l)$,  where $\alpha$ is the \textit{degree of the chain}, i.e. the maximum degree of the polynomials $P_{i,j}$, $\beta$ is the \textit{degreee of the Pfaffian function,} i.e. the degree of $P$, and $l$ is the \textit{length of the chain} is: $$(2L?,1, (\sum_{k=1}^L n_k + \sum_{k=1}^L n_k  \textrm{LengthDerivative}_k ) \cdot m  ) $$. 

% \begin{remark}



% Applying Lemma \ref{lem:network_pfaf} for instance to the sigmoid case, we obtain that the Pfaffian format of the multilayer network  is:
% $$(3L-1,1, \sum_{k=1}^L n_k \cdot m ) $$

% \end{remark}

% \begin{proof}[Proof of Theorem \ref{th:bce_loss}]
% \begin{equation*} 
% \begin{split}
% \frac{\partial L(\mathbf{\theta})}{\partial \theta_j} &=  \frac{1}{m} \frac{\partial \sum_{i=1}^m - y_i \log(f(\mathbf{\theta},x_i) - (1-y_i) \log(1-f( \mathbf{\theta} ,x_i) }{\partial \theta_j}\\
% & = \frac{1}{m}\sum_{i=1}^m  \frac{y_i}{f(\mathbf{\theta},x_i)} \frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j} + \frac{(1- y_i)}{1- f(\mathbf{\theta},x_i)} \frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j} \\
% & =  \frac{1}{m}\sum_{i=1}^m  \frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j}  \Big[ \frac{ f(\mathbf{\theta},x_i) - y_i }{ f(\mathbf{\theta},x_i)(1-  f(\mathbf{\theta},x_i))}\Big] 
% \end{split}
% \end{equation*}

% We have that the derivative of the BCE loss  is polynomial in $\frac{1}{ f(\mathbf{\theta},x_i)  } $, $\frac{1}{ 1- f(\mathbf{\theta},x_i)  } $ and  $ \frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j}$ .
% Since the derivative of the function $\frac{1}{ f(\mathbf{\theta},x_i)  } $  wrt to the parameters $\theta_j$ can be expressed as a polynomial in the function  itself  and $\frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j} $ and the same holds for $\frac{1}{ 1- f(\mathbf{\theta},x_i)  } $ to obtain a Pfaffian chain for the BCE loss we need a chain that contains all the derivatives wrt the weights, the function $f(\mathbf{\theta},x_i)$, $\frac{1}{ f(\mathbf{\theta},x_i)  } $ , $\frac{1}{ 1- f(\mathbf{\theta},x_i)  } $. Then we only need to add $\frac{1}{ f(\mathbf{\theta},x_i)  } $ , $\frac{1}{ 1- f(\mathbf{\theta},x_i)  } $ to the chain obtained in Lemma \ref{lem:network_pfaf}.
% We observe that the degree of the polynomial of the derivative of the BCE loss is $ \beta +4 $ since as seen in the Lemma  \ref{lem:network_pfaf} when the last layer is linear the function $ f(\mathbf{\theta},x_i)$ can be expressed as a polynomial of degree $\beta +1$ in
% $ ( \sigma_1(a_1^1), \dots, \sigma_{\ell}(a_1^1), \sigma_{1}(a_2^1), \dots,  \sigma_{1}(a_{n_L}^L)), \dots , \sigma_{\ell}(a_1^1) $
% . 
% We also consider that we have $m $ samples and if $f(\theta,x_i)$ will be parametric in $x_i$ and so a different function even if in the same format. It follow that the length is multiplied my $m$ while the degree of the chain and the maximum degree of the derivatives stay unaltered.
% From this it follows that the complexity of the chain is 
% $$ ( (L-2)(\beta + \alpha + \alpha(\beta +1)) + \beta +4, \beta , (\ell h(L-1) + \ell +2)m ) $$
% While when we apply the non-linearity to the last layer the complexity of the chain becomes 
% $$ ((L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \; \; \beta +3 , \; \;  (\ell h ( L- 1) + \ell   +2)m  )$$
% \end{proof}


% \begin{proof}[Proof of Theorem \ref{th:mse_loss}]
% \begin{equation*} 
% \begin{split}
% \frac{\partial L(\mathbf{\theta})}{\partial \theta_j} &= \frac{1}{m}\frac{\partial \sum_{i=1}^m (y_i - f(\theta, x_i )^2}{\partial \theta_j}\\
% & =  -\frac{2}{m} \sum_{i=1}^m (y_i - f(\theta,x_i)) \frac{ \partial f(\theta, x_i)}{\partial \theta_j} \end{split}
% \end{equation*}

% We have that the derivative of the MSE loss  is polynomial in $ f(\mathbf{\theta},x_i)   $ and  $ \frac{\partial f(\mathbf{\theta},x_i)}{\partial \theta_j}$ .
% The Pfaffian chain for the MSE loss has the same length of the Pfaffian chain of $f(\theta,x_i)$, the same maximum degree of the derivatives and the degree of the chain is the degree of the chain of $f(\theta,x_i)+1$

% The complexity of the chain for $f(\theta,x_i) $ is 

%  $$ ((L-2)( \beta + \alpha  + \alpha (\beta + 1) ) + \beta , \; \; \beta + 1, \; \;  \ell h  (L-1)  )$$ when $f(\theta,x ) = a^L$ and $$((L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \; \; \beta , \; \;  \ell h ( L- 1) + \ell_{o}    )$$ if $f(\theta,x ) = g(a^L)$.
 
 
% $$ ((L-2)(\beta + \alpha + \alpha(\beta +1)) + \beta, \beta +2 , (\ell h  (L-1))m )$$
% While when we apply the non-linearity to the last layer the complexity of the chain becomes 
% $$ ((L-2) ( \beta + \alpha + \alpha (\beta+1)) +\beta +1, \; \; \beta +1 , \; \;  (\ell h ( L- 1) + \ell_{o}    )m )$$



%\section{OLD }


% \textcolor{red}{OLD!!!}

% \subsection{$\delta_i^{L}$ for BCE loss function}




 
% Therefore, if $l<L$ the degree of the polynomial that gives $\delta^{l}_j$ (see eq (  \ref{degree_on_delta_l})) is: $$ \text{degree}(\delta^{L} )+ (1 + \text{degree}(\sigma'))(L- \ell) +  \text{degree}(\sigma) $$


%     Now, if $y_i = \sigma_i(a)$: 
% \begin{equation*}
%     \frac{d \sigma(a)}{d a} \bigg|_{a = a_h^l} =  \frac{ d Q(y_1, \dots, y_{\ell} )}{d a}\bigg|_{a = a_h^l} =  \Big(  \sum_{s= 1}^\ell \frac{\partial Q(y_1, \dots, y_\ell) }{\partial y_{s}} P_u(a, y_1, \dots, y_u) \Big) \bigg|_{
%  \begin{array}{c}
%       1\leq u \leq \ell \\
%       y_u = \sigma_u(a_h^l) \\ 
%       a = a_h^l
%  \end{array} }
% \end{equation*}

% $\frac{\partial Q(y_1, \dots, y_\ell) }{\partial y_{s}} $ has degree $ \beta_{\sigma} - 1$ and $P_u(a, y_1, \dots, y_u)$ has degree $\alpha_{\sigma} $ in $\sigma_1(a), \dots, \sigma_{\ell}(a)$. In conclusion $  \frac{d \sigma(a)}{d a} \bigg|_{a = a_h^l}  $ is a polynomial of degree $ \beta_{\sigma}  + \alpha_{\sigma} - 1 $ if, $\forall i $, $P_i$ does not depend directly on $a$, and it is  $ \beta_{\sigma}  + \alpha_{\sigma} - 1 + \alpha_{\sigma} (\beta_{\sigma} +1) $ in the general case.

% Indeed if $P_i$ depends on $a$, we have that $P(a_h^l, \sigma_1(a_h^l), \dots, a_h^l)$ has degree $\alpha_{\sigma}(\beta_{\sigma} +1)$, since the degree of $a_h^l $ is $\beta_{\sigma} +1 $ in the Pfaffian chain. 
% Notice that $a_h^l= W^l \sigma(a^{l-1})$ and $\sigma(a^{l-1})$ has degree $\beta_{\sigma} $.

% It follows that the maximum degree of the polynomial of the derivatives is $$\text{degree}(\delta^{L} )+ (1 + \alpha_{\sigma}(\beta_{\sigma} +1) )(L- 1) +  \beta_{\sigma} $$ 
% in the general case and degree 
% $$\text{degree}(\delta^{L} )+ (1 + \beta_{\sigma}  + \alpha_{\sigma} - 1 )(L- 1) +  \beta_{\sigma} $$ 
% if the polynomial $(P^i_{\sigma}(a), \sigma_1(a), \dots , \sigma_{\ell_{\sigma}}(a)) $ don't depend explicitly on $a$. 

% The degree of  $\delta^L$ depends on the chosen loss and on the format of $g$. 

% To satisfy the Pfaffian condition for all $w^l_{i,j}$ we have to include in the chain all $\sigma(a_i^l)$ for all possible $l \in \{1, \dots, L-1\}$ and respectively $i \in \{1, \dots, n_l \}$ .
% In the case where the last layer is not linear, namely $f_{\theta}(x) = g(a^L)$ we have to include the $g(a_j^L)$, if it's linear we don't need to include them.
% As a consequence, total length of the chain, for a single input point $(x_i,y_i)$,  is $  \underbrace{\ell_{\sigma} \sum_{k=1}^{L-1} n_k}_{\text{ for } \sigma \text{ and } \sigma'} +   \underbrace{\ell_g  n_L}_{\text{ for }  g}  + \underbrace{n_L}_{\text{ for the }  \text{ if we need something more } }   $ if the last layer is not linear and $ \underbrace{\ell_{\sigma}\sum_{k=1}^{L-1} n_k}_{\text{ for } \sigma \text{ and } \sigma'}  +  \underbrace{n_L}_{\text{ for the } \delta^L }   $ if the last layer is linear.
% The length of the chain and its degree will depend on the the $\delta^L$, that varies depending on the  loss we use. 
% $a^L$ of course depends on the input sample $x_i$ we will omit this dependency to keep the notation simpler. 
% We need to compute all possibles $a^l_i$ and for all possible input $x$ as argument, so we need to multiply the previous terms by $m$.

% \textbf{MSE Loss.}
% In particular, if the loss is MSE:
% \begin{align*} loss_{\text{MSE}}(f(x_i),y_i)=  \frac{1}{2}(y_i - f(\theta, x_i)  )^2.\end{align*}
% Now depending on whether the last layer is linear or the non-linearity $g$ is applied we have that 
% \begin{align*}
% \delta^L =
% \begin{cases}
%   \sum_{i=1}^m  y_i - f_{\theta}(x_i)    \text { if } f_{\theta}(x) = a^L\\
%  \sum_{i=1}^m (y_i - f_{\theta}(x_i)  )g'(a^L)  \text { if } f_{\theta}(x) = g(a^L).
% \end{cases}
% \end{align*}
% It follows that the degree of $\delta^{L}$ for the MSE loss  in the linear case is $ \beta_{\sigma}+1$ indeed we don't have $a^L$ in the chain, but $\sigma(a^{L-1})$ is included and $a^L = W^L \sigma(a^{L-1})$. 
% While in the non-linear case  the degree of $\delta^L$ is give by the degree of  $g'(a^L) g(a^L)$. Using the argument we used before for $\sigma'$, we have that the degree of $g'(a)$  is $ \beta_{g}  + \alpha_{g} - 1 $ if, $\forall i $, $P^i_{g}$ does not depend directly on $a$, and it is  $ \beta_{g}  + \alpha_{g} - 1 + \alpha_{g} (\beta_{g} +1) $ in the general case.
% In both cases we don't need to add anything to the chain for the $\delta^L$ terms.
% The degree of the polynomial of the Pfaffian function will be $2(1+\beta_{\sigma})$ for the linear case and $2 ( \beta_g )$ for the non-linear case.

%  To summarize for the MSE loss is
%  %if the last layer is linear and all $P^i_{\sigma}$ don't depend explicitly on $a$,  the format of the chain is $$( 1+\beta_{\sigma}+ (1 + \beta_{\sigma}  + \alpha_{\sigma} - 1 )(L-1)  + \beta_{\sigma}, \; 2(1+\beta_{\sigma}) , \; m \; \ell_{\sigma} \; \sum_{k=1}^{L-1} \; n_k )$$
% % $$= ( 1+2\beta_{\sigma}+ (\beta_{\sigma}  + \alpha_{\sigma} )(L-1), \; 2(1+\beta_{\sigma}) , \; m \; \ell_{\sigma} \; \sum_{k=1}^{L-1} \; n_k ).$$
% %The format 
% $$( 1+\beta_{\sigma}+ (1 +\text{degree}(\sigma'))(L-1) +\beta_{\sigma}  , \; 2(1+\beta_{\sigma}) , \; m \; \ell_{\sigma} \; \sum_{k=1}^{L-1} \; n_k )$$

% Where $$\text{degree}(\sigma')= \begin{cases}
%     \beta_{\sigma}  + \alpha_{\sigma} - 1  \; \; \text{case } 1\\ 
%    \beta_{\sigma}  + \alpha_{\sigma} - 1 + \alpha_{\sigma} (\beta_{\sigma} +1)  \text{case  }2
% \end{cases}$$ 
% Where case $1$ refers to the case where $P^i_{\sigma}(a, \sigma_1(a), \dots , \sigma_{\ell_{\sigma}}(a))$ 
% don't depend explicitly $a$ and case $2$ where they depend on it.

% While if the non-linearity $g$ is applied to the last layer, assuming the polynomials $P^i_g(a, g_1(a), \dots,g_{\ell_g}(a))$ and the polynomial of the derivatives of  the format of the chain for the loss is $$( 2\beta_g + \alpha_g -1 + (1 + \text{degree}(\sigma'))(L-1) +  \beta_{\sigma}  , \; 2  \beta_g  , \; m (\ell_{\sigma } \; \sum_{k=1}^{L-1} \;  n_k +  \ell_{g}  )   ).$$ 

% \textbf{BCE Loss.}
% For the BCE loss
% \begin{align*} loss_{\text{BCE}}(f(x_i),y_i)= - y_i  \log(f_{\theta}(x_i)) - (1-y_i)  \log(1- f_{\theta}(x_i)).\end{align*}

% Again, we assume that the polynomials $P^i_g(a, g_1(a), \dots,g_{\ell_g}(a))$ $ P^i_{\sigma}(a, \sigma_1(a), \dots,\sigma_{\ell_{\sigma}}(a))$ don't depend explicitly on $a$, so the degree of $g'$ is $\beta_g + \alpha_g -1$.
% In this case $\delta_{k}^L $ is  obtained as sum over all the samples $(x_i,y_i) $ of $\frac{\partial loss_{\text{BCE}}(y_i,f_{\theta}(x_i))}{\partial a^L}$. 
% If we consider only a single sample $x$ and the output of the network $f_{\theta}(x) = g(a^L)$. We have that 
% \begin{align}
% \label{delta_BCE}
% \frac{\partial loss_{\text{BCE}}(y,f_{\theta}(x))}{\partial a^L} =  g'(a^L)\frac{1}{g(a^L) (1- g(a^L))}(y_i - f_{\theta}(x))  =\sum_{i=1}^m  \frac{ g'(a^{L})}{g(a^L)(1-g(a^L))}(y - g(a^L)).
% \end{align}

% If the non-linearity $g$ is the sigmoid function $ \Big( g(x) = \frac{1}{1 + e^{-x}}\Big)$, the term $ \frac{ g'(a^{L})}{g(a^L)(1-g(a^L))}$ becomes $1$ and we don't need to deal with it and the degree of $\delta^L$ is the degree of $g(a^L)$, that is $\beta_g$ that for the sigmoid function is 1. We recall indeed that the sigmoid function is Pfaffian with format $(2,1,1)$.

% If the activation function is not sigmoid, we also have to add to our chain $\frac{1}{g(a^L)} $ and $\frac{1}{1-g(a^L)}$, meaning that we have to add to the chain  the fractions $\frac{1}{g}, \frac{1}{1-g}$, namely $2$ terms. Their derivatives will have degree 
% $ 2 +$ degree$(g') = 1+\beta_g + \alpha_g$.

% Considering that in binary classification the two labels are $0$ and $1$, so either $y=0$ or $y=1$. It means that in eq (\ref{delta_BCE}) one of the two terms in the denominator, $(1- g(a^L))$ and  $ g(a^L)$, can be cancelled with $y-g(a^L)$. Therefore degree of $\delta_{k}^L $ is at most $ \beta_g + 1 $.

% Whether we use a sigmoid activation function or a different activation function, in both cases we need to include in the chain the terms $\log(f_{\theta}(x_i)) $ and $\log(1- f_{\theta}(x_i)) $ and their derivatives, namely $\log(g(a^L))$ and $\log(1-g(a^L))$ for all points in the sample.
% Their derivatives will be  $\frac{g'}{g} $ or $ -\frac{g'}{1-g}$ that since we included $\frac{1}{g}$ and $\frac{1}{1-g}$ in the chain will have degree $ 1 +$ degree$(g') = \beta_g + \alpha_g$.


% Therefore for the BCE loss where the non-linearity of the last layer is sigmoid, while for all previous layers was a Pfaffian function $g$,  the format of the chain is $$( 1+ (1 + \text{degree}(\sigma'))(L-1) +  \beta_{\sigma}  , \; 1 , \;   \;  \; m \; (\ell_{\sigma}\sum_{k=1}^{L-1} \;  n_k + 3n_L ) ) .$$

% While for the BCE loss where the last layer has a non-linearity $g$ like all others layers, the format of the chain for the loss is $$ (1+ \alpha_g + 2\beta_g +  (1 + \text{degree}(\sigma'))(L-1) +  \beta_{\sigma} , \; 1 , \;   \;  \; m \; (\ell_{\sigma} \sum_{k=1}^{L-1} \; n_k +   n_L ( \ell_g + 4 ) ).$$ 
% % Where $$\text{degree}(\sigma')= \begin{cases}
% %     \beta_{\sigma}  + \alpha_{\sigma} - 1  \; \; \text{case } 1\\ 
% %    \beta_{\sigma}  + \alpha_{\sigma} - 1 + \alpha_{\sigma} (\beta_{\sigma} +1)  \text{case  }2
% % \end{cases}$$ 
% % Where case $1$ refers to the case where $P^i_{\sigma}(a, \sigma_1(a), \dots , \sigma_{\ell_{\sigma}}(a))$ 
% % don't depend explicitly $a$ and case $2$ where they depend on it.

% %The $\max$ came out, since we included also $\frac{1}{g}$ and $\frac{1}{1-g}$  in the chain their complete dervatives $ \frac{\partial \frac{1}{g(a^L}}{\partial w_{^1_{i,j}}} = \frac{1}{g(a^L)^2} g'(a^L) \frac{a^L}{\partial w^1_{i,j}} =  2 + \alpha_g,  +  (1 + \alpha_{\sigma})(L-1) $. 
% %Indeed, \textcolor{red}{(metti disegnino).....}


% \end{proof}
